A Preliminary Study of Neural Network-based Approximation for HPC Applications

Machine learning, as a tool to learn and model complicated (non)linear relationships between input and output data sets, has shown preliminary success in some HPC problems. Using machine learning, scientists are able to augment existing simulations by improving accuracy and significantly reducing latencies. Our ongoing research work is to create a general framework to apply neural network-based models to HPC applications. In particular, we want to use the neural network to approximate and replace code regions within the HPC application to improve performance (i.e., reducing the execution time) of the HPC application. In this paper, we present our preliminary study and results. Using two applications (the Newton-Raphson method and the Lennard-Jones (LJ) potential in LAMMP) for our case study, we achieve up to 2.7x and 2.46x speedup, respectively.

==> Text/comment.tex <==
\begin{comment}
From the point of view of convergence time, Newton–Raphson algorithm is not always the winner, particularly during the early stage of calculation. 
In numerical experiments, only in case that an initial assumption is close enough to the minimum, the advantage of Newton–Raphson algorithm can be fully embodied.
The iterations in Newton-Raphson method cannot be controlled, sometimes a large number of iterations must be performed to produce an adequately small residual. 
The average iteration of Newton method is around $9.44$ in $102,400$ times computation when even the initial solution given is a random range from $[1,100]$.
The running time (or iterations) of Newton-Raphson method mainly depends on the initial assumption given. 
Let $f(x)$ be a differentiable function and let $x_0$ be a guess for a solution to the equation $f(x)=0$ We can product a sequence of points $x=x_0, x_1, x_2, \dots $ via the recursive formula $$x_{n+1}=x_n-\frac{f(x_n)}{f'(x_n)}$$ that are successively better approximation of a solution to the equation $f(x)=0$.The process will be end up until either the absolute difference between two adjacent approximations is less than $E$, or the number of iterations reaches N.
If the given initial assumption is close to the final solution, the equation can be solved quickly. Otherwise, sufficient trial and error for the formula will be taken before the final solution is reached.  From the point of view of iterative convergence rate, Newton-Raphson method is strongly input data-dependent in terms of feasibility, accuracy, and convergence rate.
\end{comment}


\begin{comment}
The overall procedure of molecular simulation is illustrated in Figure \ref{fig:lj_workflow}.

 \begin{figure}[!t]
 \label{fig:lj_workflow}
    \centering
    \includegraphics[width=0.48\textwidth, height=0.30\textheight]{Figure/fig2.eps}
       \vspace{-15pt}
	    \caption{The flowchart of basic algorithm.} 
  \vspace{-15pt}
\end{figure}
\end{comment}

We use a compiler to output the corresponding inputs and outputs of a target function by the method of program instrumentation.

We observe the behavior of candidate code regions with log information of inputs and outputs(The algorithm of LJ force calculation is presented in Algorithm \ref{alg:ForceCalculation}).
Actually, just one force is involved in calculation according the Newton's third law. 

\begin{comment}
\subsection{General Results}
A single figure comparing the best NN models with the original code;


\subsection{Solution Convergence}

\subsection{The Impact of Initialization}

\subsection{Comparison with Other Machine Learning Models}
CNN vs. linear regression vs. other NN models
\end{comment}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.32\textwidth, height=0.20\textheight]{Figure/activation.pdf}
       \vspace{-15pt}
	    \caption{The tendency of training loss and test accuracy with time steps.} 
  \vspace{-5pt}
\label{fig:LAMMPS_activation}
\end{figure}

\begin{comment}
\textbf{Appropriate inputs and outputs.}
Machine learning is a data-oriented approach...
...no data-dependency beyond the code region.
...trade-off of speedup and accuracy will be count when choosing the inputs and outputs.
\end{comment}

\textcolor{blue}{(Dong's comment: the following example Soble operator is confusing and useless. You need to delete it.)}

\begin{comment}
For example, the Sobel operator is an edge detection algorithms used in image processing and computer vision. Its input may involve the various size of images, while the algorithm itself is trying to convolve the image with a small, separable, and integer-valued filter in the horizontal and vertical directions(i.e., a small $3\times3$ kernel).
In essence, the Sobel operator invokes a small $3\times3$ kernel computation iteratively, instead of executing operations on the whole input.

Small-sized inputs are more light for construction of learning-based models and improve the resulting fidelity. At the same time, the regular same-sized data is critical to model reuse and facilitate the acceleration.
A trained machine learning model is expected to give a prediction of the values of output variables. 
%even though input variables have different values from one invocation of the code region to another. 
Note that if an input or output variable changes its size (e.g., an input 2D matrix changes its size from 512x512 to 1024x1024), then the machine learning model must be re-trained.
\end{comment}

\textcolor{blue}{(Dong's comment: the above paragraph needs to be deleted.)}
\textcolor{red}{have done.}

\begin{comment}
In each iteration of the training phase, we randomly fetch $200$ samples over the full training to set and tune hyper-parameters at each iteration and use backpropagation to converge very well to local optima.

Note that the proper learning rate should be carefully tuned to gain a good convergence to a global optimum instead of local optima. 
The direction of the gradient update in SGD is not stable, which relies on a batch sample in each iteration.
Hence, we use Momentum approach, which combines the concept of momentum in physics to simulate the inertia of motion, to incorporate the previous gradients into the current update. 
\end{comment}

In order to reduce the computational cost of operations involved in the Newton–Raphson algorithm, we design an alternative machine learning (and data-driven) approach to solving the linear equations.
Because definite outputs can be acquired from the Newton-Raphson equations, we try to use a supervised neural network model to mimic the whole procedure of the Newton-Raphson method.
\textcolor{blue}{(Dong's comment: the above paragraph is too wordy. Delete it.)}

\textcolor{red}{delete: Physical parameters of the system are configured as the same.}
\textcolor{blue}{Dong's comment: what are the "physical parameters"? Confusing.}
The L-J potential is a type of short-range forces, which involves force calculation of individual pairs of atoms.
Generally, we choose to replace the code invoked frequently, and enable acquire the best rewards of speedup.

\textcolor{blue}{Dong's comment: integrate the below discussion into your above discussion. You don't need to separately list the below discussion.}
\textbf{Discussion.}
Talk about the selection of code region and inputs-outputs.
\textcolor{blue}{Dong's comment: expand the above discussion. Why do we use the combination of the two functions.}
\textcolor{red}{}


\begin{comment}
For the supervised learning, there are typically two phases: training and inference. 
During the training phase, the input to the HPC application in question is used as the input to the neural network; the output of the neural network is fine-tuned using the output of the numerical simulation model by Backpropagation~\cite{werbos1974backprop}.
We also measure the loss of the neural network across the gradient decent iterations to find the optimal solution.
During the inference process, the prediction accuracy is evaluated by the absolute error calculated by the difference between the predicted value and the ground-truth.
\end{comment}

%computational system with multiple layers and connections, which is inspired by the biological neural networks, to 
%a directed acyclic graph 

%describe some details about weight, bias, forward propagation and back propagation
%http://cs231n.github.io/neural-networks-1/
%http://ufldl.stanford.edu/tutorial/supervised/MultiLayerNeuralNetworks/
%For each single neuron, it receives input information from predecessor neurons and produces output signals along its (single) axon like a biological neuron.

%activation, the training phase and the inference phase
 
%loss and accuracy；


%\subsection{Quantification of Computation Complexity of Numerical Solver}
%Quantify the solver complexity by counting floating point numbers and memory access numbers;

==> Text/intro.tex <==
\section{Introduction}
\label{sec:intro}

%These methods include 
\textit{random fault injection}~\cite{ics12:casas, europar14:calhoun, 
 bifit+:SC12, sc16:guanpeng, prsdc13:sharma}, and to use \textit{program analysis}~\cite{asplos12:hari, isca14:hari, tdsc11:pattabiraman, prdc05:karthik, hpdc17:Calhoun} to track errors on individual instructions








